Understanding Membership Inferences on Well-Generalized Learning Models

Membership Inference Attack (MIA) determines the presence of a record in a machine learning model's training data by querying the model. Prior work has shown that the attack is feasible when the model is overfitted to its training data or when the adversary controls the training algorithm. However, when the model is not overfitted and the adversary does not control the training algorithm, the threat is not well understood. In this paper, we report a study that discovers overfitting to be a sufficient but not a necessary condition for an MIA to succeed. More specifically, we demonstrate that even a well-generalized model contains vulnerable instances subject to a new generalized MIA (GMIA). In GMIA, we use novel techniques for selecting vulnerable instances and detecting their subtle influences ignored by overfitting metrics. Specifically, we successfully identify individual records with high precision in real-world datasets by querying black-box machine learning models. Further we show that a vulnerable record can even be indirectly attacked by querying other related records and existing generalization techniques are found to be less effective in protecting the vulnerable instances. Our findings sharpen the understanding of the fundamental cause of the problem: the unique influences the training instance may have on the model.

==> tables.tex <==
%!TEX root = main.tex
\begin{table}[!t]
\centering
\caption{\fontsize{11}{13}\selectfont XXXtable2XXXXX}
\label{tab:table2}

\begin{tabular}{C{2.5cm}C{2.5cm}C{2.5cm}}
\hline
 & $1-$ precision-recall & \specialcell{recall \\ precision $\geq 0.8$} \\
\hline
\specialcell{Querying \\ the target} & $26\%$ & $30\%$ \\ \hline
\specialcell{w/o Querying \\ the target} & $4\%$ & $48\%$ \\
\hline
\end{tabular}

\end{table}



